ConneX: Automatically Resolving Transaction Opacity of Cross-Chain Bridges for Security Analysis

As the Web3 ecosystem evolves toward a multi-chain architecture, cross-chain bridges have become critical infrastructure for enabling interoperability between diverse blockchain networks. However, while connecting isolated blockchains, the lack of cross-chain transaction pairing records introduces significant challenges for security analysis like cross-chain fund tracing, advanced vulnerability detection, and transaction graph-based analysis. To address this gap, we introduce ConneX, an automated and general-purpose system designed to accurately identify corresponding transaction pairs across both ends of cross-chain bridges. Our system leverages Large Language Models (LLMs) to efficiently prune the semantic search space by identifying semantically plausible key information candidates within complex transaction records. Further, it deploys a novel examiner module that refines these candidates by validating them against transaction values, effectively addressing semantic ambiguities and identifying the correct semantics. Extensive evaluations on a dataset of about 500,000 transactions from five major bridge platforms demonstrate that ConneX achieves an average F1 score of 0.9746, surpassing baselines by at least 20.05\%, with good efficiency that reduces the semantic search space by several orders of magnitude (1e10 to less than 100). Moreover, its successful application in tracing illicit funds (including a cross-chain transfer worth $1 million) in real-world hacking incidents underscores its practical utility for enhancing cross-chain security and transparency.

==> sections/problem/3.3_terms.tex <==

\subsection{Terminology}
\label{subsec:terms}

% * 这一小节中，我们说明在本文中使用的术语(短语)。
% * transaction / transaction instance: 如前所述，每个 Transaction 会发送若干条 event log。我们把我们把一条trx和它发送的log一起称为transaction instance。在本文中，transaction和 event log通常不会分开处理，所以我们也用 "transaction"来指代 "transaction instance"
% * key, value, field: 如图2所示，解码后的transaction instance的格式表现为由键到值的映射，我们将映射的键称为"key", 值称为 "value"。同时，若将嵌套的映射看作一棵多叉树结构，则每个叶子（也就是值）都有一条唯一的从树根到自身的由非叶节点组成的路径。我们将这条路径上的所有字符串拼接起来，称为 "field". 这样，每个值都有一个唯一的field与自己对应。例如，在图2中，正确答案的field可以表示为\varname{log[CreatedOrder]-order-receiverDst}
% * key infomation(key info): 用于描述跨链交易的语义的信息。每个跨链交易中，为了方便链桥运营者记录，或者方便开发者调试，在transaction instance中会显式或隐式地存在关于这次跨链交易的语义信息。否则，链桥无法确定用户的确发起了跨链交易，用户也无法确认自己的跨链交易是否成功地实现了接收。因此，我们在 \ref{XXX}中定义了5种 key info。
% * 五元组：为了设计一个通用的方法，我们需要寻找每种 key info 与 field 之间的对应关系，所有的5个对应关系就被合称为五元组。例如，图2的例子对应的五元组就是 {to: log[CreatedOrder]-order-receiverDst, amount: log[CreatedOrder]-order-takeAmount, ...}

This section clarifies the terminology used throughout this paper.

\stitle{Transaction / Transaction Instance:} As previously mentioned, each transaction emits several event logs. We define a "transaction instance" as the combination of a transaction and its associated event logs.  Since transactions and their event logs are typically considered together within the scope of this paper, the term "transaction" will often be used as shorthand to refer to a "transaction instance."

\stitle{Key, Value, Field:} As illustrated in \figurename~\ref{fig:motivation_example}, a decoded transaction instance is formatted as a key-value mapping.  We define the "key" as the key in this mapping and the "value" as the corresponding value. Furthermore, consider the nested mapping structure as a multi-way tree. Each leaf node (representing a "value") has a unique path from the root node to itself, traversing only non-leaf nodes. The concatenation of the strings representing these non-leaf nodes along the path is defined as the "field" for that value.  Therefore, each value has a unique "field" associated with it. For example, in \figurename~\ref{fig:motivation_example}, the field corresponding to the recipient address might be represented as \varname{log[CreatedOrder].order.receiverDst}.

\stitle{Key Information (Key Info):} This refers to information that describes the semantic intent of a cross-chain transaction.  To facilitate record-keeping by chain bridge operators and debugging by developers, cross-chain transaction instances typically contain explicit or implicit semantic information related to the transaction.  Without this information, the chain bridge cannot reliably verify that a user initiated a cross-chain transfer, nor can the user confirm the successful completion of the transfer.  We define five types of "key info" in \sectionname~\ref{subsec:design_overview}.

\stitle{Quintuple:} To develop a generalized method, we aim to identify the correspondence between each type of "key info" and its corresponding "field." The set of these five correspondences is referred to as the "Quintuple"(5-tuple). For example, the quintuple for the transaction instance shown in \figurename~\ref{fig:motivation_example} might be represented as: 
\begin{lstlisting}
to: log[CreatedOrder].order.receiverDst 
chain: log[CreatedOrder].order.takeChainId
token: log[CreatedOrder].order.giveTokenAddress
amount: log[CreatedOrder].order.takeAmount
timestamp: transaction.timestamp
\end{lstlisting}


